Measurement of $W^+W^-$ production in association with one jet in proton--proton collisions at $\sqrt{s} =8$ TeV with the ATLAS detector

The production of $W$ boson pairs in association with one jet in $pp$ collisions at $\sqrt{s} = 8$ TeV is studied using data corresponding to an integrated luminosity of 20.3 fb$^{-1}$ collected by the ATLAS detector during 2012 at the CERN Large Hadron Collider. The cross section is measured in a fiducial phase-space region defined by the presence of exactly one electron and one muon, missing transverse momentum and exactly one jet with a transverse momentum above 25 GeV and a pseudorapidity of $|\eta|<4.5$. The leptons are required to have opposite electric charge and to pass transverse momentum and pseudorapidity requirements. The fiducial cross section is found to be $\sigma^{\mathrm{fid,1\textrm{-}jet}}_{WW}=136\pm6($stat$)\pm14($syst$)\pm3($lumi$)$ fb. In combination with a previous measurement restricted to leptonic final states with no associated jets, the fiducial cross section of $WW$ production with zero or one jet is measured to be $\sigma^{\mathrm{fid,}\leq\mathrm{1\textrm{-}jet}}_{WW}=511\pm9($stat$)\pm26($syst$)\pm10($lumi$)$ fb. The ratio of fiducial cross sections in final states with one and zero jets is determined to be $0.36\pm0.05$. Finally, a total cross section extrapolated from the fiducial measurement of $WW$ production with zero or one associated jet is reported. The measurements are compared to theoretical predictions and found in good agreement.

==> Makefile <==
# Makefile for creating an ATLAS LaTeX document
#------------------------------------------------------------------------------
# By default makes mydocument.pdf using target run_pdflatex.
# Replace mydocument with your main filename or add another target set.
# Adjust TEXLIVE if it is not correct, or pass it to "make new"
# Replace BIBTEX = bibtex with BIBTEX = biber if you use biber instead of bibtex.
# Adjust FIGSDIR for your figures directory tree
# Adjust the %.pdf dependicies according to your diredctory structure
# Use "make clean" to cleanup.
# Use "make cleanpdf" to delete $(BASENAME).pdf.
# "make cleanall" also deletes the PDF file $(BASENAME).pdf.

#-------------------------------------------------------------------------------
# Check which TeX Live installation you have with the command pdflatex --version
TEXLIVE  = 2013
LATEX    = latex
PDFLATEX = pdflatex
BIBTEX   = bibtex
# BIBTEX = biber
DVIPS    = dvips
DVIPDF   = dvipdf

#-------------------------------------------------------------------------------
# The main document filename
BASENAME = WW1JetPaper
#-------------------------------------------------------------------------------
# Adjust this according to your top-level figures directory
# This directory tree is used by the "make cleanepstopdf" command
FIGSDIR  = figs
#-------------------------------------------------------------------------------

# EPSTOPDFFILES = `find . -name \*eps-converted-to.pdf`
rwildcard=$(foreach d,$(wildcard $1*),$(call rwildcard,$d/,$2) $(filter $(subst *,%,$2),$d))
EPSTOPDFFILES = $(call rwildcard, $(FIGSDIR), *eps-converted-to.pdf)

# Default target - make mydocument.pdf with pdflatex
default: run_pdflatex

.PHONY: new newtexmf draftcover preprintcover auxmat \
	clean cleanpdf help

# Standard pdflatex target
run_pdflatex: $(BASENAME).pdf
	@echo "Made $<"

#-------------------------------------------------------------------------------
# If your bib files are not in the main directory adjust this target accordingly
#%.pdf:	%.tex *.bib bibtex/bib/*.bib
%.pdf:	%.tex *.tex */*.tex *.bib
	$(PDFLATEX) $<
	-$(BIBTEX)  $(basename $<)
	$(PDFLATEX) $<
	$(PDFLATEX) $<
#-------------------------------------------------------------------------------

new:
	if [ $(TEXLIVE) -ge 2007 -a $(TEXLIVE) -lt 2100 ]; then \
	  sed s/atlas-document/$(BASENAME)/ template/atlas-document.tex | \
	    sed 's/texlive=20[0-9][0-9]/texlive=$(TEXLIVE)/' >$(BASENAME).tex; \
	else \
	  echo "Invalid value for TEXLIVE: $(TEXLIVE)"; \
	  sed s/atlas-document/$(BASENAME)/ template/atlas-document.tex >$(BASENAME).tex; \
	fi
	cp template/atlas-document-metadata.tex $(BASENAME)-metadata.tex
	touch $(BASENAME).bib
	touch $(BASENAME)-defs.sty

newtexmf:
	if [ $(TEXLIVE) -ge 2007 -a $(TEXLIVE) -lt 2100 ]; then \
	  sed s/atlas-document/$(BASENAME)/ template/atlas-document-texmf.tex | \
	    sed 's/texlive=20[0-9][0-9]/texlive=$(TEXLIVE)/' >$(BASENAME).tex; \
	else \
	  echo "Invalid value for TEXLIVE: $(TEXLIVE)"; \
	  sed s/atlas-document/$(BASENAME)/ template/atlas-document.tex >$(BASENAME).tex; \
	fi
	cp template/atlas-document-metadata.tex $(BASENAME)-metadata.tex
	touch $(BASENAME).bib
	touch $(BASENAME)-defs.sty

draftcover:
	if [ $(TEXLIVE) -ge 2007 -a $(TEXLIVE) -lt 2100 ]; then \
	  sed 's/texlive=20[0-9][0-9]/texlive=$(TEXLIVE)/' template/atlas-draft-cover.tex \
	    >$(BASENAME)-draft-cover.tex; \
	else \
	  echo "Invalid value for TEXLIVE: $(TEXLIVE)"; \
	  cp  template/$(BASENAME)-draft-cover.tex $(BASENAME)-draft-cover.tex; \
	fi

preprintcover:
	sed 's/texlive=20[0-9][0-9]/texlive=$(TEXLIVE)/' template/atlas-preprint-cover.tex >$(BASENAME)-preprint-cover.tex
	#cp template/atlas-preprint-cover.tex $(BASENAME)-preprint-cover.tex

auxmat:
	sed s/atlas-document/$(BASENAME)/ template/atlas-auxmat.tex | \
	sed 's/texlive=20[0-9][0-9]/texlive=$(TEXLIVE)/' >$(BASENAME)-auxmat.tex

run_latex: $(BASENAME).dvi
	$(DVIPDF) -sPAPERSIZE=a4 -dPDFSETTINGS=/prepress ${BASENAME}
	@echo "Made $<"

# Targets if you run latex instead of pdflatex
%.dvi:	%.tex 
	$(LATEX)    $<
	-$(BIBTEX)  $(basename $<)
	$(LATEX)    $<
	$(LATEX)    $<

%.bbl:	%.tex *.bib
	$(LATEX) $*
	$(BIBTEX) $*

help:
	@echo "To create a new document give the commands:"
	@echo "make new [BASENAME=mydocument] [TEXLIVE=YYYY]"
	@echo "make"
	@echo "If your bib files are not in the main directory, adjust the %.pdf target accordingly." 
	@echo ""
	@echo "If atlaslatex is installed centrally, e.g. in ~/texmf:"
	@echo "make newtexmf [BASENAME=mydocument] [TEXLIVE=YYYY]"
	@echo ""
	@echo "If you need a standalone draft cover give the commands:"
	@echo "make draftcover [BASENAME=mydocument] [TEXLIVE=YYYY]"
	@echo "pdflatex mydocument-draft-cover"
	@echo ""
	@echo "If you need a standalone preprint cover give the commands:"
	@echo "make preprintcover [BASENAME=mydocument] [TEXLIVE=YYYY]"
	@echo "pdflatex mydocument-preprint-cover"
	@echo ""
	@echo "If you need a document for auxiliary material give the commands:"
	@echo "make auxmat [BASENAME=mydocument] [TEXLIVE=YYYY]"
	@echo "pdflatex mydocument-auxmat"
	@echo ""
	@echo "make clean    to clean auxiliary files (not output PDF)"
	@echo "make cleanpdf to clean output PDF files"
	@echo "make cleanall to clean all files"
	@echo "make cleanepstopdf to clean PDF files automatically made from EPS"
	@echo ""

%.ps:	%.dvi
	$(DVIPS) $< -o $@

clean:
	-rm *.dvi *.toc *.aux *.log *.out \
			*.blg *.brf *.bcf *-blx.bib *.run.xml \
		*.cb *.ind *.idx *.ilg *.inx \
		*.synctex.gz *~ ~* spellTmp 

cleanpdf:
	-rm $(BASENAME).pdf 
	-rm $(BASENAME)-draft-cover.pdf $(BASENAME)-preprint-cover.pdf
	-rm $(BASENAME)-auxmat.pdf

cleanall: clean cleanpdf

# Clean the PDF files created automatically from EPS files
cleanepstopdf: $(EPSTOPDFFILES)
	@echo "Removing PDF files made automatically from EPS files"
	-rm $^

